SAQAM: Spatial Audio Quality Assessment Metric

Audio quality assessment is critical for assessing the perceptual realism of sounds. However, the time and expense of obtaining ''gold standard'' human judgments limit the availability of such data. For AR&VR, good perceived sound quality and localizability of sources are among the key elements to ensure complete immersion of the user. Our work introduces SAQAM which uses a multi-task learning framework to assess listening quality (LQ) and spatialization quality (SQ) between any given pair of binaural signals without using any subjective data. We model LQ by training on a simulated dataset of triplet human judgments, and SQ by utilizing activation-level distances from networks trained for direction of arrival (DOA) estimation. We show that SAQAM correlates well with human responses across four diverse datasets. Since it is a deep network, the metric is differentiable, making it suitable as a loss function for other tasks. For example, simply replacing an existing loss with our metric yields improvement in a speech-enhancement network.

==> README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> templete/tables/ablation1.tex <==
\def\arraystretch{1.2}
\begin{table}[b!]
\large
\centering
\vspace{-0\baselineskip}
% \setlength{\tabcolsep}{2pt}
\resizebox{1\columnwidth}{!}{
 \begin{tabular}{l c c c c c}
 
 \toprule
 {\bf Name}  & {\bf \multicolumn{1}{c}{\bf HiFi}} & {\bf \multicolumn{1}{c}{\bf Dereverb}} & {\bf \multicolumn{1}{c}{\bf PEASS}} & {\bf \multicolumn{1}{c}{\bf VCC16}}& {\bf \multicolumn{1}{c}{\bf \multicolumn{1}{c}{\bf H\_{Ted}}}} \\
 \toprule
 
{\bf OURS - \emph{default}} & 0.88 & \bf 0.86 & \bf 0.39 & \bf 0.61 & 0.89 \\ 

\cdashline{1-6}
{\bf \hspace{1mm} after stage 1} & \bf 0.93 & 0.75 & 0.33 & 0.28 & \bf 0.95\\ 
\cdashline{1-6}
 
{\bf  \hspace{1mm} w/o \PESQ\, calib.} & 0.85 & 0.73 & 0.18 & 0.44 & 0.77\\ 
\cdashline{1-6}

{\bf  \hspace{1mm} same clean rec.} & 0.40 & 0.68 & 0.35 & 0.21 & 0.79 \\
{\bf  \hspace{1mm} w/o phase rep.} & 0.49 & 0.77 & 0.19 & 0.56 & 0.88 \\ 
\cdashline{1-6}

{\bf  \hspace{1mm} target \PESQ} & 0.20 & 0.59 & -0.21 & -0.12 & 0.14 \\
{\bf  \hspace{1mm} w/o stage 1} & 0.55 & 0.65 & 0.08 & 0.10 & 0.77 \\ 

 \bottomrule
\end{tabular}
}
\vspace{-0.0in}
\caption{\textbf{Ablation studies}.~Spearman correlations (SC) of our model with MOS across different ablation components are shown (Sec~\ref{ssec:ablations}).~$\uparrow$ is better.}
\vspace{-0.0in}
\label{table_ablation}
\end{table}

==> templete/text/02-background.tex <==
\section{Related work}

AMBIQUAL~\cite{narbutt2020ambiqual} was one of the first objective metrics to assess sound quality and localization of sound sources. Although useful, it had certain drawbacks:~(ii) sound quality as depending on a single channel, (iii) non-differentiable, (i) ambisonic signals, so doesnt account for factors like listening direction and influence of HRTFs used for rendering (iv) task specific (e.g, audio codecs). To overcome the last two concerns, researchers develop a task-agnostic metric BAMQ that works on binaural signals and depends on various binaural auditory cues (ITD,ILD and IACC). However, it is sensitive to background noise, and works well only under anechoic conditions - hindering their usage in diverse, realistic sound synthesis scenarios. It also assumes that the two binaural signals to be compared are time-aligned and of equal length which is not always the case. A direct comparison of our metric with BAMQ is available in section xxx.

==> templete/text/03-proposed-metric.tex <==
\section{The OURS Framework}

Our framework, \OURS\, is designed to assess the quality of a given pair of binaural signals across various attributes. In this paper, we consider two such attributes: listening quality (LQ) and spatialization quality (SQ), but the framework can be easily extended to include more attributes.
%
Given two binaural signals denoted by $x_\mathtt{1}$ and $x_\mathtt{2}$, our goal is to compute distance functions $D_1(x_\mathtt{1},x_\mathtt{2})$ and $D_2(x_\mathtt{1},x_\mathtt{2})$ that precisely characterize \listeningquality\ and \spatializationquality\ between them. The distance function is designed to be \emph{non-negative} and \emph{monotonic}, thereby making it a pseudo-metric (we do not impose triangle or associative properties).
% first propose the sound quality metric, then a combined - comprehensive metric (multi-head model), and then a single-embedding model that combines both models.
% ablation: impact of feature selection on the MOS correlations + effect on sampling rate.

\subsection{\listeningquality\ model}
\label{quality_model}
% except training, what are the features of the sound quality model
We begin by building a listening quality assessment model for binaural signals. This model processes both the magnitude and phase spectrograms of the two channels and outputs an embedding that captures the quality of that recording. It is trained using a triplet comparison dataset, in which we simulate human judgments on a simple question: ``Is A or B closer to reference C?”. We algorithmically modify clean recordings under a variety of real-life degradation's that are characteristic of degradation's commonly found in audio processing tasks including additive noises, speech distortions, binaural noise and compression across one or more sources.
% %On a high level, our model is
% presented with a triplet of samples, where one is considered
% the “anchor” and the other two consist of a “positive” and
% a “negative”, and the model is trained to map the samples
% into an embedding space where the “positive” is closer to the
% “anchor” than the “negative”, as illustrated in Figure 2(A).

% including both single channel noises applied individually to each channel of the binaural signal, as well as inherently collected binaural noise recordings. Refer to Sec (xxx).

\subsection{\spatializationquality\ model}
% DOA modelling strategies
\label{doa_modelling}
We re-purpose a model that was trained on source-localization that predicts the Direction-of-arrival (DOA) of a given sound source~\cite{manocha2021dplm}. Given a binaural input, the DOA model processes both the magnitude and phase spectrograms of the two channels, and systematically outputs a framewise
location estimate of the source. In our case, we only look at the Moving-source model that resulted in a finer resolution estimate of DOA. To improve robustness, we train DOA models with carefully designed input perturbations as data augmentations that mimic realistic environments.

% Inspired from Manocha et al.~\cite{manocha2021dplm}, we build a source-localization model that predicts the DOA of a given sound source. Given a binaural input, the DOA model processes both the magnitude and phase spectrograms of the two channels, and systematically outputs a framewise location estimate of the source. We evaluate two variants to ensure generalization of the proposed framework for realistic sound sources: a Static-Source model for recordings with a fixed source in the scene, and a Moving-Source model where the source can move smoothly in the scene. Note that the moving-source model would result in a finer resolution estimate of DOA.


\subsection{Multi-task Model}
\label{comprehensive_model}

Multi-task learning (MTL)~\cite{caruana1997multitask} has been beneficial to many speech applications~\cite{fu2016snr,chen2015multitask}. MTL aims to leverage useful information contained in multiple related tasks to help improve the generalization performance on all tasks. In our case, we consider the tasks of  listening quality prediction, and spatial localization as the two tasks for MTL. Separating the learning task into
two separate tasks is important is because the two tasks share useful common information that can be exploited. It makes the model easier to use - in the sense that if only the localization head results are needed or if only the listening quality is required, the appropriate head can be used while discarding the other one. Moreover, since MTL encourages learning shared information, even the common shared layers of the model can be used in cases where an overall estimate of quality is required rather than individual estimates of LQ and SQ.
% The other advantage is that we can throw away the two heads and only utilize embeddings for OVRL quality that reflect shared features


%To create a more comprehensive model that assess similarity between two binaural signals across various attributes, we combine our quality assessment model with DPLMs localization assessment model. We evaluate two variants of the model for two different use cases: 1) a \emph{\bf{multi-head model}} that gives an individual assessment for each attribute (i.e, localization and quality) separately, and a \emph{\bf{single-embedding model}} that combines the individual assessments of quality and localization into a single combined estimate. 

\input{templete/tables/figure1}
\subsection{Architecture}
\label{architecture}

The model architecture of both the tasks consists of 3 components: a feature extraction block, a temporal aggregation block and a task specific head - each for listening quality and localization respectively.
%
In the MTL framework, the first two blocks are shared between the two task.

%The feature-extraction block maps the input features (that are the magnitude and phase of a signal) to an embedding maintaining the temporal structure of the signal. The resulting embedding is then processed by temporal aggregation models to learn long term dependencies. The resulting hidden representations are then fed to a task-specific heads that output an listening quality embedding per frame, and a location embedding per frame for localization respectively.

For the feature-extraction block, we used an Inception styled architecture that resulted in best features. The 6-block
Inception network consists of 64 conv filters, followed by 1x1, 3x3
and 5x5 filters, leading to 3x3 max-pooling, and a 1x2 maxpool
along the frequency dimension. For the temporal aggregation block, we use Temporal Convolutional Networks (TCNs) which consists of 4 temporal blocks. Each block consists of 2 convolutional layers with a kernel size of 1x3, with each layer consisting of 32, 64, 64 and 128 channels for each of the 4 blocks respectively. We use weight normalization~\cite{salimans2016weight} along with dilated convolutions to increase the effective receptive field of our model.

For the listening quality task, we use 2 conv. layers to transform the embedding size to 64 per frame. These are then mean-pooled in the temporal dimension to get an embedding that represents the listening quality of the audio signal. For the localization task,  we divide the azimuth plane ($\in(-180^{\circ}, 180^{\circ})$) into 50 equally spaced bins, and the elevation plane ($\in(-90^{\circ}, 90^{\circ})$) into 25 equally spaced bins. It then maps the outputs from temporal aggregation to a one-hot class encoding.

%To be able to integrate the quality model with the localization model from Manocha et al., we adapt their framework to also include our sound quality model. Their proposed models comprises of three components: a feature-extraction block, a temporal aggregation block and a task specific localization block. We keep the same size of the layers for a fair comparison.
%Subsequently, the quality metric also uses the Inception block as the feature extraction block, and a small 2 linear-layer model becomes our quality assessment head.
%For the multi-head model, we share the feature extraction block, whereas for the single embedding model, we share both the feature extraction block and the temporal aggregation blocks between both the models.

%\subsection{Deep-feature distance}
%\label{deep-feature_distance}
%The hidden embeddings resulting from the proposed framework are then {\it aggregated} to compute a deep-feature distance. 
% The motivation for using several of the internal activations, instead of the final layer alone is the fact that 
% the spatial and temporal feature extraction modules of the network in Fig \ref{model_architecture} capture different attributes of the inputs. 
%Although the network is trained to predict the source location; 
%we claim that the subspace of hidden layers contains more information about estimating localization similarity between two signals.
%~This is because feature activations at different depths learn a different set of features and so computing a deep-feature distance across them combines all these different feature-similarities at different scales.
% % many different 
% % assessing localization differences in these activations thus compares many features at different audio scales.
% Since every layer of the network learns a different representation, computing a deep-feature distance across them learns a similarity metric 
%~Note that similar metrics defined using cascades of hidden representations have been shown to correlate well with human perceptual judgments 
% in both machine vision~\cite{zhang2018unreasonable} and audio~\cite{manocha2020differentiable, germain2018speech} tasks. 
% They have also been shown to be effective in training state-of-the-art representation learning algorithms without the need for prior expert knowledge~\cite{zhang2018unreasonable}.

\subsection{Loss Functions}
\label{loss_functions}

We use different losses to learn the listening quality and localization metric. 
For listening quality, we use deep metric learning with a triplet loss as the basis for learning our sound quality metric. 
%On a high level, our model is presented with a triplet of samples, where one is considered the ``anchor” and the other two consist of a ``positive” and a ``negative”, and the model is trained to map the samples into an embedding space where the “positive” is closer to the “anchor” than the “negative”. 
Formally, we define training triplets as a set $T = \{t_{i}\}_{i=1}^{N}$ where each triplet $t_i = \{x_a^i,x_p^i,x_n^i\}$ where $x_a$ is the anchor sample, $x_p$ is the positive sample and $x_n$ is the negative sample. Then, we define the triplet loss as:
\begin{equation}
L(t) = max\{ 0,D_1(x_a,x_p) - D_1(x_a,x_n) +\delta \}
\label{eqn:triplet}
\end{equation}

Here $\delta$ is the margin value to prevent trivial solutions. $D_1(x_1,x_2)$ is the deep-feature distance~\cite{manocha2020differentiable} between the full-feature activation stacks of the two audio inputs. %given by:

% \begin{equation}
% D(x_\mathtt{i},x_\mathtt{j})=\sum_l \frac{1}{T_l C_l B_l}  ||\Fmodel_l(x_\mathtt{i})- \Fmodel_l(x_\mathtt{j})||_1.
% \label{eqn:deepfeat}
% \end{equation}

%Here $\Fmodel$ is a non-linear embedding function or deep neural network (with $l$ layers) that maps the audio input to the embedding space. 
%For the given set $T$ and the embedding function $\Fmodel$, we use stochastic gradient descent to update the network weights and minimize the loss.

For the localization metric, we use the same classification formulation as Manocha et al.~\cite{manocha2021dplm}. However, instead of using smooth label cross entropy as a loss, we use the earth mover's distance (EMD), also known as the Wasserstein distance. This loss helps focus on the inter-class relationships, since the plain cross-entropy loss only focuses on the predicted ground truth class while ignoring the relationship between classes. 
%We aim to minimize the distance from the predicted distribution to the ground-truth labeled distribution.
This is especially useful if the classes are ordered since that leads to a closed form solution, which is: 
\begin{equation}
 \mbox{\bf{EMD}}^{2}(\hat{p},p) = \sum_{n=1}^{N}(\hat{P_n} - P_n)^2
\label{eqn:deepfeat}
\end{equation}
where $P_n$ is the $n$-th element of the cumulative density function of $p$. The label distribution typically follows a one-hot vector where the element 1 is at the $v$-th position if the ground truth localization falls in that intervals. Following a normal label distribution around the correct class, we use the following discrete soft label distribution compared to a one hot one:
\begin{equation}
p_n = \begin{cases}
0.4 &\text{n=v}\\
0.2 &\text{n=v$\pm$1}\\
0.1 &\text{n=v$\pm$2}\\
0 &\text{otherwise}\\
\end{cases}
\end{equation}
where $v$ is the index corresponding to the ground truth localization. Note that we also enforce continuity of the first and the last bins for the azimuth space.

% need a proper way to say that.

\subsection{Usage}
Once the network is trained, we can predict the listening quality and spatialization quality of a test input $x_1$ with respect to any provided reference $x_2$. As mentioned earlier, this reference need \textbf{not} be the matching clean reference. Given inputs $x_1$ and $x_2$, the listening quality score is obtained from the listening quality task head $F_{LQ}$ of the network $D_1(x_1,x_2)$ by computing the deep-feature distances across activation maps. Similarly, the spatialization similarity score is obtained from the localization task head $F_{SQ}$ of the network $D_2(x_1,x_2)$ by computing the deep-feature distances across activation maps.


==> templete/text/04-results.tex <==
\section{Results}





\subsection{Objective evaluations}
\label{obj_eval}
% 1. behaviour of quality metric with disentanglement, increasing noise, monotonic relationship.
% 2. localization model as not depending on content. Correlations as well.
Objectively, we compare the different metrics on (i) robustness
to content variations; (ii) clustering in learnt space; and (iii) monotonic behavior with increasing perturbation levels. Table x shows all the results.

\noindent {\bf Robust to content variations}    
To evaluate robustness of the quality model to content variations, we create a test dataset of two groups: one consisting of pairs of recordings that have the same sound quality levels (or source location) but different recording; the other consisting of pairs of recordings having different audio quality (source locations) and recordings. We calculate the common area between these normalized distributions. All models have quite low common area, suggesting that they are robust to content variations.
% Similarly, for localization, Manocha et al. already showed that DPLM is well behaved when comparing the \emph{same} audio recordings with sources at two different locations. However, its performance when comparing two different recordings with sources at two different locations is unknown. Fig x shows the localization models output when comparing two different recordings. We see that its general trend is the same as comparing two same recordings, suggesting that the model learns the spatial cues to predict location, rather than just doing a simple spectral subtraction.

\noindent {\bf Clustered Embed. Space:}     
To further evaluate the models, we also calculate the Precision of Top $K$ retrievals which measures the quality of top $K$ items in the ranked list for both our localization and quality models. Given 10 different audio qualities (source locations) - each group consisting of 100 files having the same audio quality (same location) but different recordings, we take randomly selected queries and calculate the number of correct class instances in the top $K$ retrievals. We report the mean of this metric over all queries ($MP^k$). All models have high $MP^{k=10}$ and $MP^{k=25}$ that suggests that these audio quality levels (source locations) all cluster together in the space. This also suggests that both models learns to ``disentangle'' audio quality (source locations) from content without any specific training.

% suggesting that these acoustic perturbation groups all cluster together in the learned space. This also suggests that the sound quality model learns to ``disentangle'' acoustics from content without any specific training.
% (xxx) gets $MP^{k=10}$ = 0.92 and $MP^{k=20}$ = 0.87,
\noindent {\bf Monotonicity}
To show our quality metric's monotonicity with increasing levels of noise, we create a test dataset having different audio recordings at increasing noise perturbation levels. Figure~\ref{quality} shows the distance from the quality metric as we increase the noise levels. Dots from blue to yellow show an increase in noise level from blue having the lowest noise, to yellow having the highest noise. To quantify this trend, we calculate Spearman Correlation between the distance from the metric and the perturbation levels (Table x).

Similarly, for localization, Manocha et al. already showed that DPLM is well behaved when comparing \emph{same} audio recordings with sources at two different locations. However, its performance when comparing two different recordings with sources at two different locations is unknown. Fig x shows the localization models output when comparing two different recordings. We see that its general trend is the same as comparing two same recordings, suggesting that the model learns the spatial cues to predict location, rather than just doing a simple spectral subtraction.

% \begin{figure}[t!]

% \centering
% \includegraphics[width=\linewidth]{results/localization_comparison.pdf}

% \caption{\textbf{\emph{Framewise} localization} comparison between \emph{static} and \emph{moving} source DOA models.~The \emph{moving} trajectory in split into three intervals of \emph{constant} DOA.}
% \label{compare_static_dynamic}
% \end{figure}


% \begin{figure}[t!]

% \centering
% \includegraphics[width=\linewidth]{results/onset_d.pdf}

% \caption{\textbf{\emph{Framewise} localization} comparison between \emph{static} and \emph{moving} source DOA models.~The \emph{moving} trajectory in split into three intervals of \emph{constant} DOA.}
% \label{compare_static_dynamic}
% \end{figure}


% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{results/onset_d_incor.pdf}
% \caption{\textbf{\emph{Framewise} localization} comparison between \emph{static} and \emph{moving} source DOA models.~The \emph{moving} trajectory in split into three intervals of \emph{constant} DOA.}
% \label{compare_static_dynamic}
% \end{figure}

\noindent {\bf Localization performance}
Curve showing tracking improvements from the new loss formulation + improvements from adding the quality models + show in words. Distribution of classification probs are more accurate.


\noindent {\bf Capture onset cues}
Focus on onset of speech or onset of BRIR's. We show that after removing the . The model learns to only look at the speech onset when the BRIR onset information is not available. which might be something to improve in future works.
So we investigate if IR onset is the only information that the model captures. The localization is good in the presence of onset. Removing onset, the model just looks for the onset of speech as an indicator, and the temporal structure of predictions is lost. This could also be something that can be explored in the future. 


In all these evaluations, we see that the multi-head models performs better than the individual models, thereby confirming our hypothesis that both localization and quality tasks have some shared qualities that the multi-head model takes advantage of. However, the single embedding model performs objectively worse on the tasks, since it learns an integrated embedding that combines both tasks together. As we'll see later, it correlates best with the \emph{overall} rating.


\subsection{Subjective evaluations}
\label{sub_eval}
% 1) MOS Correlations
% 2) Curves for multiple sources and moving sources correlation with graphs shown in AMBIQUAL paper (multi-head model)

We use previously published diverse third-party studies to verify that our trained metric correlates well subjective ratings with their task. We show the results of our model and compare it to \BAMQ\,~\cite{flessner2017assessment}. We  compute  the  correlation  between  the  model’s  predicted distance with the publicly available subjective ratings, using Spearman’s Rank order correlation (SC). These correlation scores are evaluated per condition where we average scores for each condition. We choose four distinct classes of available datasets for our analysis:

\begin{enumerate}[leftmargin=0.33cm]
   \item \textbf{Bil. Ambisonics - P1 and P1\textquotesingle}~\cite{ben2021binaural}:
   compares standard and bilateral spatial audio reproduction methods to compare various spherical harmonic (SH) orders across speech, castanets and guitar, but only consists of an \textit{OVRL} rating to measure quality. This dataset has two versions: with different subjects, training sessions, and different SH orders but same stimuli.
   
   \item \textbf{Sp. Microphone Array - P2}~\cite{lubeck2020perceptual}:
   compares audio quality improvements across algorithms for binaural rendering of spherical microphone array signals using music as a stimuli, across 2 rooms and 2 source positions. This dataset also consists of an \textit{OVRL} rating, and has 96 variations of test signals per subject. Consists of non sample-aligned data.
   
   \item \textbf{HpEQ - P3}~\cite{engel2019effect}:
   compares headphone equalization (HpEQ) across generic and individualised BRIR, as well as individualized, generic or no headphone equalization across speech, pink noise and guitar, and consists of ratings across \textit{OVRL}, \textit{coloration}, \textit{distance} and \textit{direction} to measure quality. These audio samples consist of very subtle differences. Consists of non sample-aligned data.
   
   \item \textbf{Bitrate Compr. Ambis. - P4}~\cite{rudzki2019perceptual}:
   assess the degree of timbral distortions introduced by compression at different ambisonic orders (1st, 3rd and 5th) across various modalities including simple scenes (vocals, castanets, glockenspiel, pink noise) and complex scenes (electronic music (EM) and acoustic music (AM)), and consists only of Perceived quality (PQ) ratings. Consists of non sample-aligned data.
\end{enumerate}

Results are displayed in Table x, in which our proposed metric has good correlation with subjective ratings. Next, we summarize with a few observations:
\begin{itemize} [leftmargin=0.33cm]
    
    \item The single embedding model obtains a high correlation with all datasets (\textit{P1, P1\textquotesingle, P2, P3}) compared to a simple addition of the two attributes for the multi-head model, suggesting that it implicitly combines features from both attributes to arrive at the OVRL rating embedding.
    
    \item Correlations across P3 are still low, but improve compared to DPLM. This suggests that we still might require human judgments to disambiguate these recordings. 
    
    %Correlation of our metric across \textit{P3} drops significantly as compared to other datasets across both localization and quality. This suggests that our metric's estimate is not robust for quite similar recordings. Since we don't train our metric in any way on human judgments, it seems a difficult task for the model to generalise to subtle audio differences that are sometimes ambiguous, and hard to tell.
    
    \item Neural-network-based metrics are more robust to non-sample aligned data - we see that most of our models perform better than the baseline on non-sample aligned audio samples in \textit{P2}, \textit{P3} and \textit{P4}.
    
    \item Compared to \BAMQ\, and DPLM, (xxx), performs better across a wide variety of tasks and perturbations, showing higher generalizability across attributes, perturbations and downstream evaluation tasks.
    
\end{itemize}

% last para on curves that are similar for moving and multi-sources from the Ambiqual paper.


\Pranay{stuff about repeating the experiments from the Ambiqual paper and superimposing the results from their paper - opus transmission losses as well - 1 para or 2 para + one graph}
Curve showing superimposition of our localization and quality metrics with their graphs from subjective ratings.

% \begin{figure}[t!]

% \centering
% \includegraphics[width=\linewidth]{results/ambiqual_single_sc.pdf}

% \caption{\textbf{\emph{Framewise} localization} comparison between \emph{static} and \emph{moving} source DOA models.~The \emph{moving} trajectory in split into three intervals of \emph{constant} DOA.}
% \label{compare_static_dynamic}
% \end{figure}


% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{results/ambiqual_multi_sc.pdf}

% \caption{\textbf{\emph{Framewise} localization} comparison between \emph{static} and \emph{moving} source DOA models.~The \emph{moving} trajectory in split into three intervals of \emph{constant} DOA.}
% \label{compare_static_dynamic}
% \end{figure}


\noindent {\bf Performance on moving sources and multiple sources}
Most of the datasets we mentioned above only have static sources with simple scenes (i.e single source). We would also like to evaluate the performance of our metric on more complex scenes where the sources are allowed to move freely around in the scene, as well as move from single point sources towards multiple point audio sources. 


% moving sources

% multiple sources (when either of them can be moving)

\begin{table*}
\centering
% \{-0.1in}
\resizebox{0.50\textwidth}{!}{
 \begin{tabular}{l l c c c c c c c c c c c c c c c c c}
 \toprule
 \multirow{2}{*}{\bf Models} & \multirow{2}{*}{\bf Attributes} &  \multicolumn{3}{c}{\bf P3 (LQ)} \\
 \cmidrule(lr){3-5}
 & & \bf Speech & \bf Pink Noise & \bf Guitar \\
 \cmidrule(lr){1-17}
 \multirow{2}{*}{\bf Pre-trained}
 & {\bf TASNET} &  0.19 & 0.20 & 0.10 \\
 & {\bf SAGRNN}  & 0.20 &  0.24 & 0.07 \\
 \cdashline{1-17}
\multirow{3}{*}{\bf Multi-head}
 & {\bf LQ} & 0.69  & 0.22 & 0.06 \\
 & {\bf PQ} & - & - & -   \\
 & {\bf OVRL (LQ+PQ)} & - & - & -  \\
 \cdashline{1-17}
 \multirow{1}{*}{\bf Single embed}
  & {\bf OVRL} & \bf - & - & - \\
  \cdashline{1-17}
  \multirow{1}{*}{\bf Baseline}
 & {\bf \BAMQ\,} & 0.42 & 0.65 & 0.08 \\
 \bottomrule
\end{tabular}
}
\caption{LQ \textbf{Subjective evaluation}: Spearman Correlation (SC). Models include: our multi-head and single embedding models, and \BAMQ\, as baseline. Localization Quality (LQ), Perceived Quality (PQ), and Overall Quality (OVRL). $\uparrow$ is better.}
\label{table_mos}
% \{-3ex}
\end{table*}


\begin{table*}
\centering
% \{-0.1in}
\resizebox{\textwidth}{!}{
 \begin{tabular}{l l c c c c c c c c c c c c c c c c c}
 \toprule
 \multirow{2}{*}{\bf Models} & \multirow{2}{*}{\bf Attributes} & \multicolumn{3}{c}{\bf P3 (PQ)}& 
 \multicolumn{6}{c}{\bf P4 (PQ)} \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-11} 
 & & \bf Speech & \bf Pink Noise & \bf Guitar & \bf Pink Noise & \bf Vocals & \bf Castanets & \bf Glocken & \bf EM & \bf AM \\
 \cmidrule(lr){1-17}
 \multirow{2}{*}{\bf Pre-trained}
 & {\bf TASNET} & 0.19 & 0.20 & \bf 0.10  & 0.45 & 0.01 & 0.20 & 0.12 & 0.61 & 0.69 \\
 & {\bf SAGRNN} & 0.20 & 0.24 & 0.07 & 0.45 & 0.14  & 0.36 & 0.19  & 0.61  & 0.72   \\
 \cdashline{1-17}
\multirow{3}{*}{\bf Multi-head}
 & {\bf LQ}  &  - & - & - &  - & - & - & - & - & - \\
 & {\bf PQ} & 0.40 & 0.36 & 0.26 & \bf 0.36 & \bf 0.893 & \bf 0.77 & \bf 0.19 & \bf 0.50 & \bf 0.78   \\
 & {\bf OVRL (LQ+PQ)} & - & - & - & -  & - & - & - & - & -  \\
 \cdashline{1-17}
 \multirow{1}{*}{\bf Single embed}
  & {\bf OVRL} & \bf - & - & - & - & - & - & - & - & - \\
  \cdashline{1-17}
  \multirow{1}{*}{\bf Baseline}
 & {\bf \BAMQ\,} & 0.42 & 0.65 & 0.08 & -0.02 & 0.36 & 0.11 & -0.05 & 0.23 & 0.18 \\
 \bottomrule
\end{tabular}
}
\caption{PQ \textbf{Subjective evaluation}: Spearman Correlation (SC). Models include: our multi-head and single embedding models, and \BAMQ\, as baseline. Localization Quality (LQ), Perceived Quality (PQ), and Overall Quality (OVRL). $\uparrow$ is better.}
\label{table_mos}
% \{-3ex}
\end{table*}


\begin{table*}
\centering
% \{-0.1in}
\resizebox{\textwidth}{!}{
 \begin{tabular}{l l c c c c c c c c c c c c c c c c c}
 \toprule
 \multirow{2}{*}{\bf Models} & \multirow{2}{*}{\bf Attributes} & \multicolumn{3}{c}{\bf P1 (OVRL)} & \multicolumn{2}{c}{\bf P1\textquotesingle (OVRL)}& \multicolumn{1}{c}{\bf P2 (OVRL)}& 
 \multicolumn{3}{c}{\bf P3 (OVRL)} \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-11} 
 & &\bf Speech &\bf Castnets & \bf Guitar & \bf Speech & \bf Castanets & \bf Music & \bf Speech & \bf Pink Noise & \bf Guitar \\
 \cmidrule(lr){1-11}
 \multirow{2}{*}{\bf Pre-trained}
 & {\bf TASNET} & 0.65 & 0.48  & 0.20 & 0.65 & 0.35 & 0.29 & 0.19 & 0.20 & \bf 0.10 \\
 & {\bf SAGRNN} & 0.72 & 0.61 & 0.21 & 0.65 & 0.40 & 0.37 & 0.20 & 0.24 & 0.07   \\
 \cdashline{1-11}
\multirow{3}{*}{\bf Multi-head}
 & {\bf LQ} &  - & -  & - & - & - & - & - & - & - \\
 & {\bf PQ} & - & -  & - & - & - & - & - & - & -   \\
 & {\bf OVRL (LQ+PQ)} & 0.86 & 0.83 & 0.74 & 0.88  & \bf 0.94 &  0.42 & 0.74 & 0.25 & 0.13  \\
 \cdashline{1-17}
 \multirow{1}{*}{\bf Single embed}
  & {\bf OVRL} & \bf 1.0 & \bf 1.0  & \bf 0.942 & \bf 1.0 & \bf 0.94 & \bf 0.63 & \bf 0.86 & 0.40 & 0.19 \\
  \cdashline{1-17}
  \multirow{1}{*}{\bf Baseline}
 & {\bf \BAMQ\,} & 0.03 & 0.83  & 0.09 & 0.52 & 0.77 & -0.17 & 0.42 & 0.65 & 0.08  \\
 \bottomrule
\end{tabular}
}
\caption{OVRL \textbf{Subjective evaluation}: Spearman Correlation (SC). Models include: our multi-head and single embedding models, and \BAMQ\, as baseline. Localization Quality (LQ), Perceived Quality (PQ), and Overall Quality (OVRL). $\uparrow$ is better.}
\label{table_mos}
% \{-3ex}
\end{table*}




\subsection{Ablations}
\label{ablations}
% 1) Variation with phase and magnitude spectrums
% 2) Variation of localization and quality with 48KHz sampling rate.
We perform ablation studies to better understand the influence of different components of our metric. We first understand the influence of different inputs to our model, and then also analyse the improvements to our model by increasing the sampling rate of the system to 48KHz.

\noindent {\bf Multi-task learning}
In this ablation, we try to assess the significance of the multi-task formulation to that predicts localization, and listening quality together. Our results show that training to predict both together results is higher performance than training two models individually; often tthe improvement is more than 30 to 40\%.

\noindent {\bf Different input feature representations}
To evaluate how the metric varies with different types of input, we train another set of models that are trained using either magnitude spectrum or phase spectrum, and compare how well do those compare with our metric that is based on both magnitude and phase spectrum features. Table x lists the MOS correlation between the multi-head version for these models across various datasets that we considered in Sec x. We observe that phase spectrum features are better correlated with subjective ratings than magnitude spectrum features. However, we also observe that our metric that takes the combination of magnitude and phase features scores the highest correlations, suggesting that it makes use of both sets of features to obtain higher correlations.

% \noindent {\bf 16KHz VS 48KHz sampling rate}
% To evaluate the impact of sampling rate on our metric, we train another set of models that are based on 48KHz compared to our models 16KHz. Table x lists the MOS correlation between both the multi-head version for these models across various datasets we considered in Sec x. We observe that the correlations for datasets \textit{P1, P1\textquotesingle, and P4}) remain similar for both types, whereas it increases slightly for P2 and P3. This is because both P2 and P3 consist of audio sources that are moving in elevation, whereas sound sources are only moving in elevation for all other datasets. Consequently, we observe an increase in elevation localization for the 48KHz model as compared to the 16KHz model. The root-mean-square error (RMSE) decreased from around 35$^{\circ}$ in the 16KHz model to around 27$^{\circ}$ in the 48KHz model. A similar trend has been observed in human elevation localization as well. Best et al.~\cite{best2005role} studied the accuracy with which human listeners can localize spoken words. They found out that lower frequencies below 8 kHz are known to be sufficient for accurate speech recognition in most situations, these results demonstrate that natural speech contains information between 8 and 16 kHz that is essential for accurate localization.

% 1) We perform ablation studies to better understand the influence of different inputs to our metric in Table x for both models (combined and single embedding with MOS) - do not need to show all curves, just a few curves\\

% 2) change sampling rate to 48K, and show some improvements in MOS correlation across P2 and P3 (since those have elevation changes) - don't need to show all figures, just a few curves. Not much change in other datasets, but some minor change in elevation perception datasets.


\subsection{Binaural speech enhancement}
\label{enhancement}
 
% 1) comparing log MSE with our metric; subjective and objective results 'training with single-embedding model'

% describe the binaural SE model, ip op, layers and so on.
To further demonstrate the effectiveness of our metric, we design a binaural speech enhancement model that is based on a popular U-Net type convolutional neural network~\cite{tan2019learning}. The input to the model is the real and imaginary components of the STFT of the binaural signal, and the outputs are the complex ratio mask. 
%The model consists of a multi-layer convolutional encoder and decoder with U-net skip connections, and a sequence modeling network applied on the encoders output. The encoder (and decoder) consists of 5 gated convolutional layers with sigmoid activation for the gating mechanism with 2 $\times$ 6 kernels and batch normalisation. The sequence modeling network takes the encoders output and outputs a non-linear transformation of the same size. Since we design a \emph{causal} model, the LSTM network consists of 2 uni-directional lstm layers with 256 hidden units in each layer.

%The complex mask for each channel (L or R) is predicted individually. For predicting the R (or L) channel, we use the L (or R) channel as a concatenated conditional input to the model. Hence, the model takes as input 4 channels and outputs one complex mask corresponding to which channel input was placed first in the order.

The baseline enhancement model is trained on Log Mean Square Error (LogMSE) between the estimated and target real and imaginary STFT components. We supplement our loss model in two different ways: (i) LogMSE + OURS from scratch; and (ii) Finetune OURS where we first pretrain on LogMSE and finetune on OURS.

%by following the GAN training strategy, where our speech enhancement model becomes the generator, and our multi-head model becomes the discriminator / evaluator. This approach is quite similar to MetricGAN~\cite{} that proposed a similar GAN framework by training a monaural speech enhancement model on surrogate ``black-box'' discriminators that are learnt from data, and are directly related to evaluation metrics of interest (PESQ, STOI etc.,)

%The Generator ($G$) is trained to map noisy binaural speech $x$ to a corresponding clean speech $y$ by minimizing:

% \begin{equation}
%  L_{G} = \mathbb{E}_{x} [\lambda(D(x,G(x),y)) + |\mathbb{G(x)}-y|_2]
% \label{eqn:deepfeat}
% \end{equation}
% where $G(x)$ refers to enhanced speech, and $D$ is the discriminator. Since our quality network is based on a triplet loss formulation, we pass three inputs to $D$ - the target $y$ becomes the anchor, the enhanced $G(x)$ is the positive, and the noisy input $x$ becomes the negative. The first term in Eq.x is called adversarial loss for fooling $D$ weighted with a factor $\lambda$. The goal of $D$ is to distinguish between real data and generated data by minimizing the following loss function:
% \begin{equation}
%  L_{D} = \mathbb{E}_{x,y} [D(x,G(x),y))]
% \label{eqn:deepfeat}
% \end{equation}
% A lower value of $L_D$ suggests that $D$ is correctly able to identify the input noisy from the enhanced output.

% The description of the entire training procedure is in Fig x.

% \begin{algorithm}
%     \caption{Binaural Speech Enhancement Training Procedure}\label{euclid}
%     \hspace*{\algorithmicindent} \textbf{Input:} Paired clean and noisy recordings, triplet perturbation dataset discussed in Sec x , Models $D$, $G$, $k$ - the number of steps to apply to the discriminator, and $m_G$ and $m_D$ - minibatch size for $G$ and $D$ respectively \\
%     \hspace*{\algorithmicindent} \textbf{Output:} Trained models $G$ and $D$
%     \begin{algorithmic}[1]
%     \For{number of training iterations}
%     \For{k steps}
%     \State Sample mini-batch of $m_D$ triplets from current and previous checkpoints, and the triplet perturbation dataset.
%     \State Update discriminator ($D$) using Eqn x
%     \EndFor
%     \State Sample mini-batch of $m_G$ pairs from the SE data
%     \State Update generator ($G$) by minimizing Eqn x
%     \EndFor
%     \end{algorithmic}
%     \end{algorithm}

%framework for speech enhancement. They trained
% Describe our training metric
\input{templete/tables/se_models}


For evaluation, we randomly select 500 unseen audio recordings from the an unseen dataset. Following prior works, we evaluate the quality of enhanced binaural recordings using a variety of objective measures. For the objective measures, we use: i) PESQ (from 0.5 to 4.5); (ii) Short Time Objective Intelligibility (STOI) (from 0 to 100); (iii) L2 ; (iv) SI-SDR; and v) Multi-scale STFT all evaluated over each channel individually, and then averaged to get one single value.

%For subjective studies, we perform A/B preference tests internally, consisting of Ours vs baseline pairwise comparisons. Each pair is rated by x different subjects and then majority voted to see which method performs better per utterance. As shown in Fig x, our models outperform the baseline in both categories. All results are statistically significant with $p < x$.

% training params ?
% ip features, and other training parameters, plus loss function




% \subsection{Binaural synthesis using our metric}
% \label{synthesis}

% % 1) adding our 'localization' loss to the objective conviently
% % describe the binaural SE model, ip op, layers and so on.
% We show the utility of our trained metric as a loss function for the task of rendering binaural sounds from mono audio.
% We use the current state-of-the-art model by Gebru et al.~\cite{}. The model takes as input a monaural (single channel) signal, and a conditioning temporal signal that represents the position and orientation of source and listener, and  outputs a binaural (stereophonic) signal. The models consists of 3 components: (i) an encoder mapping the input signal into a learnt frequency space; (ii) a left-right masking temporal convolutional network; and (iii) a decoder mapping the translated signal back into the wave domain. Instead of simple additive or concatenated conditioning, they used a hyper-convolution layer to conditioning the network on position and orientation. The direction-dependent weights and biases obtained from the adaptor network that takes as input the direction code and outputs the weights and bias, are directly used in the temporal convolutional layers.


% The original model was trained on multi-scale STFT using STFT sizes (2048, 1024, 512, 256) with 75\% overlap. We supplement our metric in two ways: (i) train from scratch using a combination of multi-resolution STFT and our single-embedding model as an additional loss; and (ii) down-project the view vector embedding from the adaptor network, and force it close together with the embeddings from our localization model. % maybe a small picture to describe it better

% We train the model using Adam with a batch size of 98.
% The initial learning rate is $1e^{-4}$ with $\beta_1=0.9$ and $\beta_2 = 0.999$. We anneal the learning rate by a factor of two if five epochs have passed without improvement in the validation set. We train with a
% frame size of 8000 audio samples at 48kHz with 50\% overlap, with
% a frame size of 20 samples for the corresponding direction code.

% This model is trained on the Hearsay binaural audio dataset which contains a total of 2.6 hours of paired mono and echoic binaural audio from 8 different speakers. Participants were asked to walk around a mannequin and talk (no script was used), and their position and orientation were tracked.

% We randomly select 500 unseen audio recordings from the Hearsay dataset to evaluate the results. We evaluate the quality of synthesized binaural recording using both objective and subjective measures. For the objective measures, we use: i) PESQ (from 0.5 to 4.5) and (ii) Short Time Objective Intelligibility (STOI) (from 0 to 100). 

% For subjective studies, we perform A/B preference tests internally, consisting of Ours vs baseline pairwise comparisons. Each pair is rated by x different subjects and then majority voted to see which method performs better per utterance. As shown in Figx, our models outperform the baseline in both categories. All results are statistically significant with $p < x$. Overall, both our models outperform the baseline. Our 2nd model performs better than the 1st model, since these are huge models, and updates can be small per iteration. Forcing the update at the right layer speeds up training, leads to better results in shorter training.

% \begin{table}[h!]
% \resizebox{\columnwidth}{!}{ 
%  \begin{tabular}{l c c c c c | c}
%  \toprule
%  {\bf } &  {\bf \PESQ} & {\bf STOI} & {\bf CSIG} & {\bf CBAK} & {\bf COVL} & {\bf MOS}
%   \\ \toprule
%   {\bf Noisy} 
%  &  1.97 & 91.50 & 3.35 & 2.44 & 2.63 & 2.61 \\
%  \midrule
%   {\bf DEMUCS~\cite{defossez2020real}} 
%  &  3.01 & 95.00 & 4.39 & 3.44 & 3.73 & 3.73\\
%   {\bf DEMUCS+\OURS\ } 
%  & \bf 3.10 & \bf 95.07 & \bf 4.46 & 3.55 & \bf 3.82 & 3.86 \\
%  {\bf Finetune \OURS\ } 
%  & 3.06 & 94.93 & 4.30 & \bf 3.56 & 3.70 & \bf 4.07\\
%  \bottomrule
% \end{tabular}
% }
% %\{-0.10in}
% \caption{{\bf Evaluation of synthesis} models using the VCTK~\cite{valentini2017noisy} test set with four objective measures and one subjective measure.}
% %\{-2ex}
% \label{table_denoising}
% \end{table}

==> templete/text/experimental.tex <==
# Claims for the paper

1) Earlier spatialization metric; now a combined metric that estimates spatialization, and sound quality assessment model

2) Evaluate various strategies: 1) individual models 2) Combined models (common branches); and 3) entire same model ( w/ added linear layer at the end)
Main model is the multi-head model, however we can show other models in ablation sections

3) Evaluation: MOS correlation
4) Objective evaluation: a) content invariance; b) clustered embedded space; c) monotonicity; d) localization performance; e) capture onset cues

Ablations: 1) importance of mag or phase spectrum as inputs
2) 16k VS 48k trained models; 3) utility of multi-task models (show that actually lead to improvement)

Speech Enhancement
